Tool-as-Interface: Learning Robot Policies from Observing Human Tool Use

Tool use is essential for enabling robots to perform complex real-world tasks, but learning such skills requires extensive datasets. While teleoperation is widely used, it is slow, delay-sensitive, and poorly suited for dynamic tasks. In contrast, human videos provide a natural way for data collection without specialized hardware, though they pose challenges on robot learning due to viewpoint variations and embodiment gaps. To address these challenges, we propose a framework that transfers tool-use knowledge from humans to robots. To improve the policy's robustness to viewpoint variations, we use two RGB cameras to reconstruct 3D scenes and apply Gaussian splatting for novel view synthesis. We reduce the embodiment gap using segmented observations and tool-centric, task-space actions to achieve embodiment-invariant visuomotor policy learning. We demonstrate our framework's effectiveness across a diverse suite of tool-use tasks, where our learned policy shows strong generalization and robustness to human perturbations, camera motion, and robot base movement. Our method achieves a 71\% improvement in task success over teleoperation-based diffusion policies and dramatically reduces data collection time by 77\% and 41\% compared to teleoperation and the state-of-the-art interface, respectively.

==> tables/camera_pose_ablation.tex <==
\begin{table}[h!]
\centering
\caption{Policy Robustness to Camera Pose in Hammer Task. The compared methods include: (1) Ours w/o random cropping and w/o view augmentation, (2) Ours w/ random cropping and w/o view augmentation, and (3) Ours w/ random cropping and w/ view augmentation.}
\label{tab:robust_cam_pose}
\begin{tabular}{@{}l@{\hspace{5mm}}c@{}}
\toprule
\textbf{Methods}                                   & \textbf{Success Rate} \\ \midrule
Ours w/o random cropping, \newline w/o view augmentation         & 0/18                \\ 
Ours w/ random cropping, \newline w/o view augmentation          & 3/18                \\ 
Ours w/ random cropping, \newline w/ view augmentation           & 15/18               \\ \bottomrule
\end{tabular}
\end{table}


==> tables/demo_collection.tex <==

\begin{table}[h!]
\centering
\caption{Demonstration Collection Time and Success}
\label{tab:collection_times}
\begin{tabular}{@{}llcc@{}}
\toprule
\textbf{Task}            & \textbf{Collection Method} & \textbf{Time per Episode (s)} & \textbf{Can Be Collected} \\ \midrule
Meatball Scooping        & Spacemouse                & 40                            & Yes                       \\
                         & Human Hand                & 4                             & Yes                       \\ \midrule
Hammering                & Spacemouse                & 30                            & Yes                       \\
                         & Gello                     & 20                            & Yes                       \\
                         & Human Hand                & 5                             & Yes                       \\ \midrule
Pan Flipping             & Spacemouse                & $\infty$                      & No                        \\
                         & Gello                     & $\infty$                      & No                        \\
                         & Human Hand                & 1                             & Yes                       \\ \bottomrule
\end{tabular}
\end{table}


==> tables/embodiment_seg.tex <==
\begin{table}[h!]
\centering
\caption{Effects of Embodiment Segmentation}
\label{tab:embod_seg}
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Task}   & \textbf{Method}                                      & \textbf{Success Rate (Completed/Total)} \\ \midrule
Wine Balancing          & Ours with embodiment segmentation &  8/10                      \\
                & Ours without embodiment segmentation    &    0/10                                     \\ \bottomrule
Playing Soccer          & Ours with embodiment segmentation &  6/10                     \\
                & Ours without embodiment segmentation    &    2/10                                     \\ \bottomrule

\end{tabular}
\end{table}


